SemSup: Semantic Supervision for Simple and Scalable Zero-shot Generalization

Zero-shot learning is the problem of predicting instances over classes not seen during training. One approach to zero-shot learning is providing auxiliary class information to the model. Prior work along this vein have largely used expensive per-instance annotation or singular class-level descriptions, but per-instance descriptions are hard to scale and single class descriptions may not be rich enough. Furthermore, these works have used natural-language descriptions exclusively, simple bi-encoders models, and modality or task-specific methods. These approaches have several limitations: text supervision may not always be available or optimal and bi-encoders may only learn coarse relations between inputs and class descriptions. In this work, we present SemSup, a novel approach that uses (1) a scalable multiple description sampling method which improves performance over single descriptions, (2) alternative description formats such as JSON that are easy to generate and outperform text on certain settings, and (3) hybrid lexical-semantic similarity to leverage fine-grained information in class descriptions. We demonstrate the effectiveness of SemSup across four datasets, two modalities, and three generalization settings. For example, across text and image datasets, SemSup increases unseen class generalization accuracy by 15 points on average compared to the closest baseline.

==> sections/02_methods_old.tex <==
\section{Methodology}
\label{sec:methodology}

%%%%% Definitions %%%%%
\newcommand{\model}[0]{$\mathcal{M}_{\theta}$}
\newcommand{\ppred}[0]{$P_{pred}(y|x_i)$}
\newcommand{\psup}[0]{$P_{\textrm{\supervised{}}}(y|x_i)$}
\newcommand{\psemsup}[0]{$P_{\textrm{\semsup{}}}(y|x_i)$}
% \newcommand{\semout}[0]{$\mathcal{O}^{\textrm{\semsup{}}}$}
\newcommand{\mcal}[1]{\mathcal{#1}}

\newcommand{\scenarioenum}[2]{\textbf{#1#2}}
%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Background}
\label{sec:methodology:background}
Standard supervised learning (\supervised{}) uses a train dataset to learn a model which can classify an input into a fixed set of classes.
Formally, let $x_i$ and $y_i \in \mcal{Y} = \{1, \dots, K\}$ denote the input and the categorical output,
and \ppred{} be the model's prediction.
The model consists of (1) an input encoder $f(\cdot)$ and (2) an output matrix, whose $i^{\textrm{th}}$ row ($\mathcal{O}[i]$) is a representation for the $i^{\textrm{th}}$ class.
\begin{align}
    \begin{split}
        &f(x_i) \in \mathbb{R}^d, \mathcal{O} \in \mathbb{R}^{K\times d}\\
        &\textrm{\ppred} = \textrm{softmax} \left ( \mathcal{O} f(x_i)\right )
    \end{split}
\end{align}

\subsection{Semantic Supervision}
\label{sec:methodology:semsup}
The supervised learning setting (\supervised{}) ignores semantic information by using a randomly initialized output matrix to represent the classes.
Our approach (\semsup{}) addresses this shortcoming through:
(1) multiple semantically-rich class descriptions,
(2) flexible formats to describe classes (natural language and structured formats), and
(3) incorporating both lexical and semantic similarity between class descriptions and the input.

\paragraph{Multiple class descriptions} In contrast to prior works which use only the class name~\cite{frome2013devise} or a single description~\cite{bujwid2021large,qiao2016less}, \semsup{} relies on multiple semantically rich descriptions to gain a thorough understanding of a class. These descriptions can reference different attributes to provide a holistic understanding of classes.
For example, the class \textit{sports} can be described in terms of its
(a) definition (\textit{``Competitive physical activity''}),
(b) examples (\textit{``Examples include football, tennis, and cricket''}),
(c) etymology (\textit{``Derived from the Old French word desport, meaning leisure''}) and so on.

\paragraph{Alternative supervision formats} While text has been the de facto choice for class descriptions, for certain datasets describing classes in structured formats is easier than natural language.
For example, the class \textit{tiger} can be described as a JSON: \texttt{\{skin: [fur, stripes],color: [orange, black…\}}.
\semsup{} is able to flexibly utilize descriptions in any form.
We provide examples of class descriptions of different forms (text and JSON) in Appendix~\ref{sec:example_descriptions}, and details on how we collect them in \symbolsecref{sec:output_sup}.

Formally, both for natural language and structured descriptions, we define $\mathcal{C} = \left ( \mathcal{C}_1, \dots, \mathcal{C}_K \right )$ to be the descriptions for $K$ classes, where $\mathcal{C}_j = \{ c_{j1}, \dots, c_{jL} \}$ contain a set of $L$ descriptions describing the $j^{\textrm{th}}$ class.

\paragraph{Hybrid lexical-semantic similarity}
We propose two bi-encoder architectures which measure the compatibility between an input instance and class description -- (1) \semsupbi{} which uses only semantic similarity and (2) \semsupcoil{} which uses a hybrid lexical-semantic similarity model.
For both models, for each batch during training, we uniformly and independently sample a description $c_j \in \mathcal{C}_j$ for each class $j$ and encode it using an encoder $g(c_{j})$.

For an input $x_i$, \semsupbi{} uses the dot-product between the class description representation $g(c_{j})\in \mathbb{R}^{d_{out}}$ and input representation $f(x_i)\in \mathbb{R}^d$ as class logits. We add a projection matrix $\mathcal{P}$ to ensure that the dimensions match. %($\mathcal{P} \in \mathbb{R}^{d_{out} \times d}$).

\begin{align}
    \label{eq:methodology:summary}
    \begin{split}
        \textrm{\supervised{} logits}&\coloneqq \mathcal{O}[i]\:  f(x_i) \\
        \textrm{\semsupbi{} logits}&\coloneqq g(c_{j})^{\top}\mathcal{P} \: f(x_i) \\
    \end{split}
\end{align}

While \semsupbi{} can learn semantic similarity, it ignores lexical cues which are strong indicators of compatibility.
For example, for the input \textit{``Michael Jordan was \underline{competitive}''} and class \textit{``sports''} with the description \textit{``A \underline{competitive} physical activity or game''}, the common word \textit{competitive} is important to identify similarity.
To incorporate this information, we propose \semsupcoil{} motivated by~\citet{gao2021coil}. \semsupcoil{} incorporates lexical similarity using the dot-product of the contextualized representations of lexically identical words between input and outputs.
Concretely, for input $x_i$ and class description $c_{j}$, let $f_{x_i}(w)$ and $g_{c_{j}}(w)$ be the contextualized representation of a common word $w \in x_i \cup c_{j}$ (e.g., \textit{competitive}). The logits for \semsupcoil{} are:
\begin{align}
    \begin{split}
        &\textrm{{\small \semsupcoil{} logit}} := \\
        &g(c_{j})^\top\mathcal{P} f(x_i) + \sum_{w \in x_i\:\cup\:c_{j}} f_{x_i}(w_i)^\top g_{c_{j}}(w_i) \\
    \end{split}
\end{align}
To utilize \semsupcoil{} for image inputs, we construct a natural language sentence by obtaining image annotations like the color, shape, or background of the object ($\bar{x}_i$).
\semsupcoil{} uses the image instance and class description to measure semantic similarity, but the image annotations and the description for lexical and semantic similarity.
Formally, let $h(\cdot)$ be the image annotation encoder, the \semsupcoil{} logits are given by the sum of the (1) image and description semantic similarity, (2) image annotation and description semantic similarity, and (3) image attributes and description lexical similarity:
\begin{align}
    \begin{split}
    &g(c_{j})^\top\mathcal{P} \: f(x_i) + g(c_{j})^\top \mathcal{P}_I \:h(\bar{x}_i)  + \\
    &\sum_{w \in \bar{x}_i\:\cup\:c_{j}} h_{\bar{x}_i}(w_i)^\top g_{c_{j}}(w_i)
    \end{split}
\end{align}

where $\mathcal{P}_I$ is a projection matrix between image attribute and class description representations. To the best of our knowledge, we are the first to use a hybrid lexical-semantic similarity model to improve zero-shot generalization.

\paragraph{Training and testing}
During training, we learn the input encoders $f(\cdot)$, $h(\cdot)$ class description encoder $g(\cdot)$, and label projection matrices $\mathcal{P}$, $\mathcal{P}_I$ together.
Class descriptions are sampled uniformly and independently at random for each batch during both training and testing. At test-time, we predict the class corresponding to the class description with the highest softmax probability. \footnote{We found that changing random samples did not significantly change the overall accuracy on the evaluation sets.}

\paragraph{Usefulness of \semsup{}}
Intuitively, \semsup{} makes predictions over output choices by `reading' their `description' and deciding the best match for the input instance.
This is akin to training models to answer \textit{informative} multiple-choice questions, which provides several flexible use cases during inference:
(1) new unseen choices can be specified using corresponding descriptions,
(2) the number of choices can be dynamic,
and
(3) classes can be described in different ways based on end user preference,

%Thus, \semsup{} allows the model to generalize to unseen outputs and have a potentially unbounded output space into which it can classify.


\subsection{Collecting output supervision}
\label{sec:output_sup}

\semsup{} uses multiple semantically rich descriptions for generalizing to unseen classes.
We consider two kinds of descriptions -- (a) natural language and (b) structured (in JSON format), which we collect in a semi-automated fashion.
Our pipeline enables collecting descriptions of both modalities for any dataset with minimal effort.

\label{sec:setup:supervision}
\paragraph{Natural language supervision}
We collect textual class descriptions by converting class names into queries: ``what is a \textit{class}'' and issuing them to two popular search engines\footnote{\url{www.google.com} and \url{www.duckduckgo.com}}.
We scrape the resulting preview snippets, automatically remove scraper artifacts and partial descriptions, and manually filter any remaining off-topic descriptions.
\footnote{We do not manually filter RCV1 descriptions due to a large number of descriptions and classes.}
We present example descriptions in Appendix~\ref{sec:example_descriptions}.

\myparagraph{Structured supervision (JSON)}
For some datasets, supervision is easier to specify in a structured format.
We collect and provide supervision in a JSON format to evaluate its usefulness.
The JSONs contain attribute-value pairs for each class, with different datasets having their own attributes.
When class attributes are available (AWA2), we directly use them in the JSON (e.g., {\tt \{color:[orange, black]\}} for a tiger).
When class attributes are not available (RCV1, 20NG, CIFAR) we automatically construct the JSON by scraping dictionary definitions, hyponyms, and hypernyms from WordNet \cite{miller1995wordnet} and related terms from thesauri~\cite{PowerThesaurus}.
To increase description diversity, we automatically augment the descriptions by permutations and randomly dropping out values.
%We provide examples in Appendix~\ref{sec:example_descriptions}.

\paragraph{Generating image attributes}
To enable \semsupcoil{}'s use of lexical similarity on image datasets, we obtain image attributes from an object detector \cite{kolesnikov2020bigtransfer}, convert them to comma separated text, and append them to the template \textit{``This photo contains:''}.
We ensure that the list of attributes do not contain information about the ground truth class of the image by omitting detections that overlap with the class name, synonyms, or hyponyms.
Synonyms and hyponyms are removed with the help of WordNet synsets and hierarchy respectively.
